Fair PCA, One Component at a Time

The Min-Max Fair PCA problem seeks a low-rank representation of multi-group data such that the the approximation error is as balanced as possible across groups. Existing approaches to this problem return a rank-$d$ fair subspace, but lack the fundamental containment property of standard PCA: each rank-$d$ PCA subspace should contain all lower-rank PCA subspaces. To fill this gap, we define fair principal components as directions that minimize the maximum group-wise reconstruction error, subject to orthogonality with previously selected components, and we introduce an iterative method to compute them. This approach preserves the containment property of standard PCA, and reduces to standard \pca for data with a single group. We analyze the theoretical properties of our method and show empirically that it outperforms existing approaches to Min-Max Fair PCA.

==> bisection.tex <==

\begin{algorithm}[t]
\caption{Bisection Method for Problem~\ref{prob:par_eigenpair}}
    \label{alg:bisection}
\textbf{Input}: \A, \B, \tA, \tB, tolerance $\epsilon$ \\
\textbf{Output}: $\mu$ such that $q(\parv)=0$
\begin{algorithmic}[1]
     \STATE Initialize $\mu_s \gets 0$, $\mu_e \gets 1$, $\mu_m \gets \frac{1}{2}$  
     \STATE $\quadratic{m} \gets \ComputeQuadratic(\mu_m, \tA, \tB)$
    \WHILE{$|\quadratic{m}| \geq \epsilon$}
    \STATE $\quadratic{e} \gets \ComputeQuadratic(\mu_e, \tA, \tB) $
     \IF{ $\quadratic{m} \times \quadratic{e} < 0$ }
        \STATE $\mu_s \gets \mu_m$
    \STATE $\quadratic{s} \gets \ComputeQuadratic(\mu_s, \tA, \tB) $
    \ELSIF{ $\quadratic{m} \times \quadratic{s} < 0$ }
     \STATE $\mu_e \gets \mu_m$
     \ENDIF
     \ENDWHILE
     \STATE \textbf{return} $\mu_m$
\end{algorithmic}
\end{algorithm}




==> bisection_subroutine.tex <==
\begin{algorithm}[t]
\caption{\ComputeQuadratic}
    \label{alg:subroutine_bisection}
	\textbf{Input: $\mu$ , \tA, \tB } \\
        \textbf{Output: $\quadratic{\mu}$}
    \begin{algorithmic}[1]
        \STATE $U', \Sigma', V'^T \gets SVD( \mu \A^T A + (1-\mu) B^T B)$ 
        \STATE $x \gets V'^T[0,:]$ 
        \STATE $\quadratic{\mu} \gets x^T \A^T \A x - x^T \B^T \B x - \tA  + \tB$ 
        \STATE \textbf{return} $\quadratic{\mu}$
\end{algorithmic}
\end{algorithm}


==> defines.tex <==
%\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}

% DISALLOWED PACKAGES
% \usepackage{authblk} -- This package is specifically forbidden
% \usepackage{balance} -- This package is specifically forbidden
% \usepackage{color (if used in text)
% \usepackage{CJK} -- This package is specifically forbidden
% \usepackage{float} -- This package is specifically forbidden
% \usepackage{flushend} -- This package is specifically forbidden
% \usepackage{fontenc} -- This package is specifically forbidden
% \usepackage{fullpage} -- This package is specifically forbidden
% \usepackage{geometry} -- This package is specifically forbidden
% \usepackage{grffile} -- This package is specifically forbidden
% \usepackage{hyperref} -- This package is specifically forbidden
% \usepackage{navigator} -- This package is specifically forbidden
% (or any other package that embeds links such as navigator or hyperref)
% \indentfirst} -- This package is specifically forbidden
% \layout} -- This package is specifically forbidden
% \multicol} -- This package is specifically forbidden
% \nameref} -- This package is specifically forbidden
% \usepackage{savetrees} -- This package is specifically forbidden
% \usepackage{setspace} -- This package is specifically forbidden
% \usepackage{stfloats} -- This package is specifically forbidden
% \usepackage{tabu} -- This package is specifically forbidden
% \usepackage{titlesec} -- This package is specifically forbidden
% \usepackage{tocbibind} -- This package is specifically forbidden
% \usepackage{ulem} -- This package is specifically forbidden
% \usepackage{wrapfig} -- This package is specifically forbidden



\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{problem}{Problem}
%\newtheorem*{problem*}{Problem}
\newtheorem{definition}{Definition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remark}{Remark}
\newtheorem{property}{Property}
\newtheorem{proof}{Proof}

\usepackage{xcolor} % This package is necessary for coloring text
\newcommand{\mcReview}[1]{{#1}}

%% tight spacing in item lists
\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  {  \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{2em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em}
} }
\newcommand{\squishlisttight}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em}
} }

\newcommand{\squishdesc}{
 \begin{list}{}
  {  \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em}
} }

\newcommand{\squishend}{
  \end{list}
}


%\newcomman{\note}[1]}{{\textcolor{red}{\bf Note: \it #1}}}

%\newcommand{\note}[1]{}

%%%%%%%%%%%%%% compact paragraph titles
\newcommand{\spara}[1]{\smallskip\noindent{\bf #1}}
\newcommand{\mpara}[1]{\medskip\noindent{\bf #1}}

%%%%%%%%%%%%%% complexity
\newcommand{\np}{{\sc NP}\xspace}
\newcommand{\bigO}{{\sc O}\xspace}

%%%%%%%%%%%%%%%%% Algorithms
%\SetKwComment{Comment}{// }{}

\newcommand{\ie}{i.e.\xspace}
%%%%%%%%%%%%%% math symbols

\newcommand{\reals}{\ensuremath{\mathbb R}\xspace}


\newcommand{\ssq}{\ensuremath{\lambda_{\max}}}
\newcommand{\parv}{\ensuremath{\mathbf{v}(\mu)}}
\newcommand{\parl}{\ensuremath{\mathbf{\lambda}(\mu)}}

\newcommand{\lagrangian}{\ensuremath{\mathcal{H}}}
\newcommand{\vecspace}{\ensuremath X}
\newcommand{\seenvecspace}{\ensuremath\tilde \vecspace}
\newcommand{\users}{\ensuremath\mathcal U}
\newcommand{\seenusers}{\ensuremath\tilde{\mathcal U}}
\newcommand{\items}{\ensuremath\mathcal R}
\newcommand{\seenitems}{\ensuremath\tilde{\mathcal R}}
\newcommand{\expected}[1]{\ensuremath\mathbb E\left[#1\right]}
\newcommand{\bfb}{\ensuremath{\mathbf{b}}\xspace}
\newcommand{\bfr}{\ensuremath{\mathbf{r}}\xspace}
\newcommand{\matrixR}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\matrixX}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\matrixY}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\matrixI}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\matrixM}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\Ait}{\ensuremath{\mathbf{A}_i^{\top}\mathbf{A}_i}\xspace}
\newcommand{\bfA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\bfV}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\bfW}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\bfU}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\bfQ}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\bfP}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\matrixC}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\bfs}{\ensuremath{\mathbf{s}}\xspace}
\newcommand{\bfone}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\bfx}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}\xspace}
\newcommand{\bfq}{\ensuremath{\mathbf{q}}\xspace}



\newcommand{\datamatrix}{\ensuremath{{X}}\xspace}
\newcommand{\datacolumn}{\ensuremath{{x}}\xspace}

\newcommand{\VV}{\ensuremath\mathcal V}
\newcommand{\groups}{\ensuremath\mathcal G}
\newcommand{\vc}{\ensuremath{\bfv^{\perp}}}
\newcommand{\Vc}{\ensuremath{\bfV^{\perp}}}


\newcommand{\bfmu}{\ensuremath{\boldsymbol{\mu}}\xspace}
\newcommand{\bfv}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\bfw}{\ensuremath{\mathbf{w}}\xspace}
\newcommand{\trace}{\ensuremath{\mathit{Tr}}\xspace}
\newcommand{\rank}{\ensuremath{\text{rank}}\xspace}

\newcommand{\scaledvs}{\ensuremath{{D}}\xspace}

\newcommand{\nullvector}{\ensuremath{\mathbf{0}}\xspace}


%%%%%%%%%%%%%%%% problem defines
\newcommand{\MINMAX}{{\sc MinMax}\xspace}
\newcommand{\svd}{{\sc SVD}\xspace}
\newcommand{\maxcut}{{\sc MAX-CUT}\xspace}

\newcommand{\ngroups}{\ensuremath{k}\xspace}


%\newcommand{\cnote}[1]{}fbox{{\bf Note:} #1}}

\newcommand{\cnoteokhm}{\cnote[OK HM]{}}

% PCA
\newcommand{\pca}{{\sc PCA}\xspace}
%\newcommand{\fairpca}{{\sc FairPCA}\xspace}
\newcommand{\QR}{{\sc QR}\xspace}
\newcommand{\RRQR}{{\sc RRQR}\xspace}
\newcommand{\HRRQR}{{\sc H-RRQR}\xspace}
\newcommand{\LRRQR}{{\sc L-RRQR}\xspace}

% CSS problems
\newcommand{\css}{{\sc CSS}\xspace}
\newcommand{\cssminmax}{{\sc CSS-MinMax}\xspace}
\newcommand{\faircss}{{\sc FairCSS}\xspace}
\newcommand{\faircssminmax}{{\sc FairCSS-MinMax}\xspace}
\newcommand{\faircssmorethank}{{\sc FairCSS-BoundedError}\xspace}
\newcommand{\minfairnessscores}{{\sc MinFairnessScores}\xspace}
\newcommand{\dualminfairnessscores}{{\sc MinFairnessScores-Dual}\xspace}
\newcommand{\twominfairnessscores}{{\sc 2-MinFairnessScores}\xspace}
\newcommand{\kfairnessscores}{{\sc $c$-FairnessScores}\xspace}
\newcommand{\lscore}[2]{{\ensuremath \ell_{#2}^{(k)}(#1)}}
\newcommand{\maxloss}{{\sc MaxLoss}\xspace}

\newcommand{\maxL}{\text{Max} {\ensuremath \mathcal{L} }\xspace}
\newcommand{\maxLArgs}[2]{\text{Max}   {\ensuremath \mathcal{L}(#1, #2)}\xspace}

\newcommand{\loss}{{\ensuremath {\mathcal{L}} }\xspace}

\newcommand{\ksubsetsum}{{\sc $k$-SubsetSum}\xspace}

\newcommand{\slowqr}{{\sc S-Low QR}\xspace}
\newcommand{\shighqr}{{\sc S-High QR}\xspace}
\newcommand{\sgreedy}{{\sc S-Greedy}\xspace}
\newcommand{\lowqr}{{\sc Low QR}\xspace}
\newcommand{\highqr}{{\sc High QR}\xspace}
\newcommand{\greedy}{{\sc Greedy}\xspace}
\newcommand{\random}{{\sc Random}\xspace}
\newcommand{\sampler}{{\sc FairScoresSampler}\xspace}


\newcommand{\communities}{{\sf\small communities}\xspace}
\newcommand{\communitiesfour}{{\sf\small communities-4}\xspace}
\newcommand{\compas}{{\sf\small compas}\xspace}
\newcommand{\compasthree}{{\sf\small compas-3}\xspace}
\newcommand{\adult}{{\sf\small adult}\xspace}
\newcommand{\german}{{\sf\small german}\xspace}
\newcommand{\recidivism}{{\sf\small recidivism}\xspace}
\newcommand{\student}{{\sf\small student}\xspace}
\newcommand{\meps}{{\sf\small meps}\xspace}
\newcommand{\heart}{{\sf\small heart}\xspace}
\newcommand{\credit}{{\sf\small credit}\xspace}

\newcommand{\gaussianthree}{{\sf\small gaussian-3}\xspace}

\newcommand{\opt}{{\sf\small opt}\xspace}
\newcommand{\minmax}{{\sf\small minmax}\xspace}
\newcommand{\fair}{{\sf\small fair}\xspace}
%
%\newcommand{\mc}[1]{#1}
\newcommand{\mc}[1]{{#1}}

%
\newcommand{\A}{\ensuremath{{A}}\xspace}
\newcommand{\B}{\ensuremath{{B}}\xspace}
%
\newcommand{\tA}{\ensuremath{t_{A}}\xspace}
\newcommand{\tB}{\ensuremath{t_{B}}\xspace}
%

\newcommand{\rankoneloss}{{$1$-Dimensional Loss}\xspace}

\newcommand{\lossOneD}{{\loss_{\text{1-D}}}\xspace}

\newcommand{\lossIncremental}{{\loss_{\text{incr}}}\xspace}


\newcommand{\guassian}{{\sf\small gaussian}\xspace}

\newcommand{\fairPCA}{{\sc
Fair \pca}\xspace}


% quadratic 
\newcommand{\quadratic}[1]{\ensuremath{Q_{#1}}\xspace}


% subroutine 
\newcommand{\ComputeQuadratic}{\textsc{ComputeQuadratic}\xspace}

% problems
\newcommand{\fairsvdextended}{{\sc Fair Principal Components}\xspace}
\newcommand{\fairsvd}{{\sc Fair PCs}\xspace}
\newcommand{\faireig}{{\sc Fair-PC}\xspace}
\newcommand{\dual}{{\sc FAIR-PC-Dual}\xspace}

%% algorithms 
%\newcommand{\fairsvd}{Fair-SVD\xspace}
\newcommand{\fairsvdfw}{{\sc \fairsvd-FW}\xspace}
\newcommand{\fairpca}{{\sc FAIR-PCA}\xspace}
\newcommand{\fairpcaalgo}{{\sc FAIR-PCA-SDP}\xspace}
\newcommand{\bicriteria}{{\sc Bicriteria}\xspace}

\newcommand{\sdp}{{\sc SDP}\xspace}
\newcommand{\sdps}{{\sc SDP}s\xspace}
%\newcommand{\twofairsvd}{{\sc 2-FairSVD}\xspace}



==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

%\cnote{this section is work in progress}
This section presents our experimental evaluation, 
%describes the experimental setup, the datasets, and gives 
%the results of the experimental evaluation 
%carried out to evaluate the proposed methods.
%of our methods.
%The goal of
which aims at assessing the performance of 
%More specifically, the goal of the  experiments is to 
%demonstrate the benefits of 

the our method (Algorithm \ref{alg:fairsvd}) in its quintessential application: fair principal component analysis. Exploring other applications is left to future work. We refer to the multigroup singular vectors output by Algorithm \ref{alg:fairsvd} as \fairsvd. 

The experiments consider both the two-group case, where our methods are supported by optimality guarantees, and the case of more than two groups, where we observe that, in practice, the gap between primal and dual solutions is consistently small and hence they are close to optimal.  
%We carry out experiments first in the standard two-group scenario, where the algorithms are supported by theoretical guarantees. We also evaluate our algorithms in the general case of more than two groups, where we do not have theoretical guarantees. In this case, we evaluate the empirical duality gap, and we observe that in practice our solutions are close to optimal.
 %the algorithm based on the Frank-Wolfe optimization framework.  
 %which is the algorithm of choice in this setting. 
%¤\cnote[HM]{Could one replace the two sentence in the above paragraph by just referring to the algorithms by name? Or do we need the sentences at all?}
%\cnote[MC]{We do not really have a name for the algorithm tailored to the two-group setting, it is not given so much space. The other one can be referred to as Algorithm~\ref{pseu:FW}}
%\cnoteokhm
%InThe this experiments, we focus on the variant of our methods based on the Frank-Wolfe method. 
The results also show that our method can offer significant advantages over the recent \fairpca method~\cite{tantipongpipat2019multi}.
%Specifically, while \fairpca preserves fairness only in the subspace of the target dimension given as input, as we show, \fairsvd preserves fairness in every subspace. Additionally, \fairsvd
%drastically reduces the runtime of \fairpca, while  achieving comparable reconstruction quality.  

\subsection{Settings}\label{sec:settings}
Next, we illustrate the datasets, metrics, baselines, parameter settings and experimental setup used in our experiments. 

\spara{Datasets.} 
\begin{itemize}[noitemsep, topsep=0pt]
    \item \textbf{Datasets with two groups,} We use the juvenile recidivism data (\recidivism) from
Catalunya~\cite{tolan2019machine} 
%and medical expenditure survey data 2015
%(\meps)~\cite{cohen2009medical} 
and various datasets from the UCI
machine learning repository~\cite{dua2019uci}: "heart-cleveland" (\heart),
 "german-credit" (\german), "credit-card" (\credit), "student
performance" (\student), "adult" (\adult), "compas-recidivism" (\compas), "communities"
(\communities).  Group membership is based on sex, except for "\communities" where groups determined by racial composition (caucasian majority or not).

%one group consists of communities with a "caucasian" majority (i.e., at least $50\%$ of the community members are "caucasian"), whereas the other group consists of communities with a "non-caucasian" majority.  

%where groups are based on either a
%majority white (i.e., at least $50\%$ of the community members are white) or a non-white community (i.e., at least $50\%$ of the community members are "black", "hispanic" and "asian"). 

\item \textbf{Datasets with more than two groups.} We consider the "compas-recidivism” dataset partitioned into three groups
%of approximately equal size 
according to age (\compasthree), and the "communities" dataset partitioned into four groups, namely "blacks", "hispanics", "asians" and "caucasians",  according to the dominant ethnicity (\communitiesfour). 
\end{itemize}


%and on two datasets, namely \compas and \communities. 
%For the former, we consider three groups of approximately equal size, each corresponding to a different age range. For the latter, we split the data into four groups of communities according to whether they are of "black", "hispanic", "asian" or "caucasian" prevalence. 
Data are processed by removing protected attributes, one-hot encoding categorical variables, and standardizing columns.
Table~\ref{table:dataset-stats} shows
summary statistics of the datasets.
 

\iffalse 
\begin{table}[t]
\caption{Dataset statistics. $m_A$ and $m_B$ are the number of instances in groups
$A$ and $B$, respectively. $n$ is the number of columns.}
\label{table:dataset-stats}
\centering
\begin{scriptsize} % or \small
\begin{tabular}{l r r r r r r}
\toprule
Dataset & Columns ($n$) & $m_A$ & $m_B$ & rank($A$) & rank($B)$\\
\midrule
      \heart &     14 &     201 &      96 &     13 &     13 \\
     \german &     63 &     690 &     310 &     49 &     47 \\
     \credit &     25 & 18\,112 & 11\,888 &     24 &     24 \\
    \student &     58 &     383 &     266 &     42 &     42 \\
      \adult &    109 & 21\,790 & 10\,771 &     98 &     98 \\
     \compas &    189 &  9\,336 &  2\,421 &    167 &     73 \\
\communities &    104 &  1\,685 &     309 &    101 &    101 \\
 \recidivism &    227 &  1\,923 &     310 &    175 &    113 \\
      \meps  & 1\,247 & 18\,414 & 17\,013 & 1\,217 & 1\,200 \\
%        APS-failure &   60\,000 &    171 & 59\,000 &  1\,000 \\
%          MEPS-2016 &   34\,655 & 1\,941 & 18\,129 & 16\,526 \\
\bottomrule
\end{tabular}
\end{scriptsize} % or \small
\end{table}



\begin{table}[t]
\caption{Experiments with more than $2$ groups. Dataset statistics.}
\label{table:dataset-stats-multiple-groups}
\centering
\begin{scriptsize} % or \small
\begin{tabular}{l r r r}
\toprule
Dataset & $|G|$ & \# Instances & Rank \\
\midrule
 \compas &  3 & 241, 240, 238 & 115, 110,  97 \\
\communities & 4 &  90, 1\,571, 218, 115  & 90
, 99, 103, 103 \\ 
\bottomrule
\end{tabular}
\end{scriptsize} % or \small
\end{table}
\fi 


\begin{table}[t]
\caption{Dataset statistics. For each dataset, we report the number of columns ($n$), the number of groups ($|\mathcal{G}|$), and the number of rows and rank by group.}
\label{table:dataset-stats}
\hspace*{-0.3cm} % Adjust the value to move it more or less to the left
\centering
\begin{tiny} % or \small
\begin{tabular}{l r r r r}
\toprule
Dataset & Columns ($n$) & $ | \mathcal{G} | $ & Group Rows & Group Ranks  \\
\midrule
      \heart &     14 & 2 & 201, 96 &   13,  13 \\
     \german &     63 &  2 & 690, 310 &   49,47 \\
     \credit &     25 & 2 & 18\,112, 11\,888 &   24, 24 \\
    \student &     58 & 2 & 383, 266 & 42, 42 \\
      \adult &    109 & 2 & 21\,790, 10\,771 & 98, 98 \\
     \compas &    189 & 2 & 619, 100 & 165, 71 \\
\communities &    104 & 2 & 1\,685, 309 & 101, 101 \\
 \recidivism &    227 & 2 &  1\,923, 310 &   175, 113 \\
%      \meps  & 1\,247 & 2 & 18\,414, 17\,013 & 1\,217, 1\,200 \\
%        APS-failure &   60\,000 &    171 & 59\,000 &  1\,000 \\
%          MEPS-2016 &   34\,655 & 1\,941 & 18\,129 & 16\,526 \\
 \compasthree & 189 & 3 & 241, 240, 238 & 115, 110, 97 \\
\communitiesfour & 104 & 4 &  90, 1\,571, 218, 115  & 90, 99, 103, 103 \\ 
\bottomrule
\end{tabular}
\end{tiny} % or \small
\end{table}

\spara{Metrics and parameters.}\label{sec:metrics_parameters}
To evaluate the performance of the algorithms under evaluation, we monitor the marginal loss (\mc{introduced by \citet{tantipongpipat2019multi}})\inote{Added this because there seems not be anymore an explanation of the marginal loss in the main text}, incremental loss, discussed in Section~\ref{sec:overview}, 
and
%, in order to carry out a comparison independent of the particular metric being optimized, we also monitor 
the standard $L_2$ reconstruction loss. 
We show the variation of each loss in the groups as a function of the (target) reconstruction rank $d$, which we vary from $1$ to $8$. Finally, we measure runtimes in seconds. 

%as a function of rank in the different groups

\spara{Baselines.}\label{sec:baselines}
We compare against \fairpca ~\cite{tantipongpipat2019multi}. Given target rank $d$, \fairpca returns a rank-$d$ projection matrix $\bfP=\bfU\Lambda\bfU^\top$,  where $\bfU \in \reals^{n\times d}$ is obtained through \svd (or eigendecomposition). In our experiments, we evaluate the consistency property by comparing the loss when using $\bfU_{:d}$ of \fairpca against $\bfV_{:d}$ retrieved by Algorithm \ref{alg:fairsvd}, for all possible values of the rank $d$. 

%In our experiments we 
%In our experiments, we focus on assessing the performance of \fairsvd against the recent \fairpca method. 

%We assess the performance of \fairsvd against the recent \fairpca method~\cite{tantipongpipat2019multi}.




%In order to measure the cost of enforcing balanced error across groups, for the reconstruction loss, we additionally compare against the standard \svd (\textsc{SVs}), which does not take groups into consideration. 

\spara{Experimental setup.}
Our implementation is written in \texttt{python}. 
In the two-groups case, the singular vectors for multigroup data are obtained by the tailored algorithm based on the root-finding procedure, while
 for more than two groups, they are obtained by the Frank-Wolfe algorithm.
 

%We use \texttt{numpy},
%\texttt{scipy} and \texttt{scikit-learn} for preprocessing, linear algebra
%operations as well as parallelization. The
Experiments are executed on a compute
node with 32 cores and 256GB of RAM. The (anonymized) source code is available online~\footnote{\url{https://anonymous.4open.science/r/multigroupSVs-F716/}}. 
%All reported results are averages over three repetitions.


\subsection{Results for two-group data}\label{sec:exp_results}


\begin{figure*}
\centering
 \hspace*{0.3cm}\includegraphics[width=0.375\textwidth]{images/plots/legend_SVs2.pdf} \\
    \begin{tabular}{ccc}
        \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_marginal_loss_v7.pdf} & 
        \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_incremental_loss_v5b.pdf} & 
        \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_reconstruction_error_v5d.pdf} \\
         \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_marginal_loss_multiple_groups_v4.pdf} &  \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_incremental_loss_multiple_groups_v4.pdf} &  \hspace*{-0.3cm}\includegraphics[height=0.1275\textheight]{images/plots/compas_reconstruction_error_multiple_groups_v4d.pdf} \\
    \end{tabular}
    \caption{\compas dataset with two groups (top) and \compasthree dataset with three groups (bottom). Marginal, incremental, and reconstruction loss by rank. Different marker symbols indicate different groups.}
    \label{fig:peeformance}
\end{figure*}


Figure~\ref{fig:peeformance} (top) shows the different losses incurred by our method and \fairpca in the \compas datasets as a function of the target rank $d$. 
Due to the space limitations, analogous results for all the other datasets are presented in the appendix (Figure~\ref{fig:performance_appendix}). 
%For each dataset, we report marginal loss, incremental loss and reconstruction error in both groups as a function of reconstruction rank. 
All the metrics under consideration are never significantly worse for \fairsvd than for \fairpca. 
Furthermore, the figure highlights the crucial advantage of \fairsvd: the incremental loss is the same in both groups for all values of the rank parameter lower than the input target rank ($8$ in the experiments), meaning that fairness is also pursued in the lower-dimensional subspaces. 
The incremental loss is considerably smaller for \fairsvd
%than for \fairpca
. On the other hand, the marginal loss optimized by \fairpca is never significantly smaller for \fairpca than for \fairsvd, but tends to be smaller for \fairsvd. 
Finally, the reconstruction loss is consistently comparable for \fairpca and \fairsvd. Unlike the incremental and marginal losses, the reconstruction loss can be highly different in the two groups since both \fairsvd and \fairpca do not seek to balance the reconstruction loss, but rather the distance to the best possible approximation.  %achieved by the \svd. 


%it does not consider the comparison with the best level of approximation that can be achieved 



%The reconstruction error can be significantly  different in the two groups since it does not consider the best possible approximation that can be achieved in the groups 


%We first show the clear advantages of the proposed methods in terms of runtime. 
%\spara{Runtimes.} 
In addition,
%to the comparison of the three losses under consideration
Table~\ref{tab:runtimes} shows the runtime of \fairsvd and \fairpca in the different datasets. 
While the semi-definite program proposed by Tantipongpipat et al.~\cite{tantipongpipat2019multi} becomes slow as dataset size increases, \fairsvd is generally faster, often by orders of magnitude. 

\iffalse 
\cnote[HM]{It would be better to start by results on performance, and only after that talk about runtime. So perhaps the two paragraphs can be interchanged.}

\cnote[HM]{Term "performace" often refers to computational effort. Could we replace it by "accuracy, as measured by three different loss functions, marginal loss, incremental loss, and reconstruction loss"?}
\cnote[MC]{Yes for both observations. Performance is not appropriate here, we could use just "loss" or e.g. "accuracy" or "projection quality"...}
\cnoteokhm
\fi 

\iffalse
\begin{table}[t!]
\tiny
\centering
\caption{Runtimes of different algorithms (in seconds). NA indicates that the algorithm does not terminate in a time window of $12$ hours. }
\begin{tabular}{lccc}
\toprule
Dataset & \fairsvdfw & \fairsvd & \fairpca \\
\midrule
 \heart & 0.06 & 0.009 & 0.022 \\
 \german & 0.468 & 0.104 & 0.896\\
 \credit & 0.207 & 0.229 & 0.084 \\ 
 \student & 0.317 & 0.067 & 0.64 \\
 \adult  & 2.18 & 2.157 & 9.125 \\
 \compas & 2.257 & 0.71 & 143.148 \\
 \communities & 0.868 & 0.278 & 8.623 \\
 \recidivism & 3.46 & 1.28 & 357.594\\
  \meps & & 211.124 &  NA \\
\bottomrule
\end{tabular}
\label{tab:runtimes}
\end{table}
\fi 


\begin{table}
\scriptsize
\centering
\caption{Runtimes of \fairsvd and \fairpca (in seconds) in all datasets ($d=8$). }
%NA indicates that the algorithm does not terminate within $12$ hours. }
\begin{tabular}{lrr}
\toprule
Dataset &  \fairsvd & \fairpca \\
\midrule
 \heart &  0.009 & 0.022 \\
 \german &  0.1 & 0.9\\
 \credit & 0.23 & 0.084 \\ 
 \student & 0.067 & 0.64 \\
 \adult  & 2.16 & 9.13 \\
 \compas  & 0.71 & 143.15 \\
 \communities & 0.28 & 8.62 \\
 \recidivism & 1.28 & 357.59 \\
 \compasthree & 2.54 & 124.11  \\
 \communitiesfour & 1.23 & 11.16 \\ 
%  \meps & 211.124 &  NA \\
\bottomrule
\end{tabular}
\label{tab:runtimes}
\end{table}


%The reconstruction error for the \svd in the two groups is generally considerably smaller, indicating that requiring a 




\iffalse
\begin{table*}
\centering   
\includegraphics[width=0.6\textwidth]{images/plots/legend_with_svs_sc.pdf}\\
 \begin{tabular}{ccc}
\hspace*{-0.3cm}\includegraphics[width=0.33\textwidth]{images/plots/compas_marginal_loss_v7.pdf} & \hspace*{-0.3cm}\includegraphics[width=0.33\textwidth]{images/plots/compas_incremental_loss_v5b.pdf} & \hspace*{-0.3cm}\includegraphics[width=0.33\textwidth]{images/plots/compas_reconstruction_error_v5b.pdf} \\
%\vspace*{-0.3cm}
\caption{\compas dataset with two groups. Marginal, incremental and reconstruction loss by reconstruction rank in the groups. Different marker symbols indicate different groups.}
\end{tabular}
%\label{fig:peeformance} 
\end{table*}


\begin{table*}[t]
    \centering   \includegraphics[width=0.9\textwidth]{images/plots/legend_multigroup.pdf}\\
   % \includegraphics[width=0.3\textwidth]{.pdf} & \includegraphics[width=0.3\textwidth]{.pdf}
    \begin{tabular}{ccc}
        %\midrule
        &  \heart & \\  
    \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/heart_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/heart_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/heart_reconstruction_error_v2.pdf} \\
        &  \german & \\ 
        \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/german_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/german_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/german_reconstruction_error_v2.pdf} \\
        &  \credit & \\  
        \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/credit_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/credit_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/credit_reconstruction_error_v2.pdf} \\
        &  \student & \\ 
        \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/student_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/student_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/student_reconstruction_error_v2.pdf} \\
        &  \adult & \\  
        \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/adult_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/adult_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/adult_reconstruction_error_v2.pdf} \\
        &  \compas & \\  \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/compas_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/compas_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/compas_reconstruction_error_v2.pdf} \\
        &  \recidivism & \\  
        \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/recidivism_marginal_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.12\textheight,keepaspectratio]{images/plots/recidivism_incremental_loss_v2.pdf} & \includegraphics[width=0.3\textwidth,height=0.11\textheight,keepaspectratio]{images/plots/recidivism_reconstruction_error_v2.pdf} 
        \\
        %\bottomrule
    \end{tabular}
    \caption{Real-world datasets with two groups. Marginal, incremental and reconstruction loss by rank.}
    \label{fig:peeformance}
\end{table*}
\fi 

\input{multiple_group_experiments}

==> formulation.tex <==

\section{Problem Formulation}
\label{sec:formulation}

We begin with some intuition. % behind our formulation. 
Given a matrix $\matrixM \in \reals^{m \times n}$ partitioned into $|\groups|=\ngroups$ groups, we consider the problem of finding a sequence of $d$ vectors such that each vector is orthogonal to the previous ones and minimizes the maximum loss incurred when projecting the data from any group onto such vector.
In other words, the problem asks for an orthonormal basis of a subspace where the maximum projection error across all groups is minimized. 
%\cnote[AM]{I this sentence is a nice summary but misses the consistency property of the vectors.}
Additionally, we require consistency, i.e.,  all prefixes of the sequence of vectors satisfy this condition.

The problem we consider is a natural multigroup extension of the problem of finding the first $d$ singular vectors. 
If the data forms a single group, the target vectors are exactly the (standard) singular vectors. In the remainder of this section, we discuss the details of the problem formulation. 

The idea of minimizing the maximum per-group loss is inspired by the multigroup framework of~\citet{tantipongpipat2019multi}.
The aggregated loss for a matrix $\matrixM$, partitioned into \ngroups groups, cannot decrease unless the highest per-group loss decreases. 
%\cnote[AM]{Perhaps we could say a few more words here instead of just deferring to tanti et al.}


%In particular, we explain the criteria adopted to evaluate the quality of a given sequence of vectors. 

\spara{Loss function.} % or objective? 
%Before proceeding to the problem formulation, it is necessary to introduce 
We start by introducing the per-group loss function $\loss: \VV_d \rightarrow \reals$ used to evaluate the quality of a given solution for a single group $\bfA \in \groups$. As discussed above, the global loss function for the entire %obtained by aggregating the per-group values of $\loss$ by taking the maximum. 
matrix $\matrixM$ is then simply the maximum value of $\loss$ in the groups.

The choice of the function $\loss$ is motivated by non-trivial observations, which are discussed next. Due to space limitations, however, we defer most of the details of this discussion to the appendix. 
%Next, we discuss the choice of the loss function $\loss$.

%\cnote[AM]{I think the following paragraph is too long and tedious. Was the previous version too vague?}


%Therefore,
%To overcome these limitations 
%we propose a loss function that is tailored to our setting. %and satisfies , for every $\bfv_d \subset \bfV$. 

\begin{definition}[\rankoneloss]
    Given a matrix $\bfA \in \reals^{a \times n}$ and a vector $\bfv \in \reals^n$. 
    %matrix $V \in \reals^{n \times d}$. Let $A_d$ be the component of $A$ in the orthogonal complement of $V_{:d-1}$, with $A_1=A$. 
    The $1$-dimensional loss is:
    \[
\lossOneD(\bfA,\bfv)\triangleq\sigma_1^2(\bfA)- \|\bfA\bfv\bfv^\top\|_F^2.
    \]
\label{def:one_dimensional_loss}
\end{definition}
The \rankoneloss compares the norm of the projection of $\bfA$ onto vector $\bfv$ to the best possible rank-$1$ projection norm, given by $\sigma_1$. 
%Unlike the marginal loss, the \rankoneloss is always non-negative.
%satisfies
%$\loss(\bfA,\bfv_d) \geq 0$. 

Given the \rankoneloss, 
it is straightforward to compute the total loss of a solution $\bfV$ to Problem \ref{prob:fairsvd},  using Property \ref{property:projection}. We refer to this total loss as \emph{Incremental
Loss}.
\begin{definition}[Incremental
Loss]
\label{lemma:total_loss}
Let $\bfV \in \reals^{n \times d}$ be an orthogonal matrix. The Incremental Loss is:
\[
\lossIncremental(\bfA,\bfV)\triangleq\sum_{i=1}^d \lossOneD(\bfA,\bfv_i). 
%\ssq(\bfA_i) - \|\bfA_i\bfv_i\bfv_i^\top\|_F^2 
\]
\end{definition}
\cnote[HM]{I'm not sure I understand this: if one plugs in from Definition 1, then each member of the sum over different values of i has the term $\sigma^2_1(A)$. A few lines later there is $\sigma_1(A_i)$?}
Notice that $\lossIncremental$ attains its minimum at zero. 
The minimum is achieved by setting, for all $i$, $\bfv_i$ to the right singular vector of $\bfA_i$ associated with $\sigma_1(\bfA_i)$, which provides the best possible rank-$1$ approximation for $\bfA_i$.
%Thus it is more well-behaved than $\loss_{\text{marg}}$ for \fairsvd. 
As we will illustrate, this simple observation is crucial to prove the optimality of the algorithm we give for the case $|\groups|=2$.

\iffalse 
\begin{observation}
\label{obs:minzero}
    $\min \lossIncremental(\bfA,\bfV)=0$.
\end{observation}

 %the optimality of that singular vector as the best rank-1 approximation for $\bfA_i$. 
\fi 

\spara{Comparison with other loss functions.} The most commonly used loss function for \svd and \pca is the reconstruction error. However, in the multigroup setting where the per-group errors are aggregated by the maximum operator, the reconstruction error suffers from an important limitation. 
Intuitively, it may be possible to perfectly reconstruct some groups in a $d$-dimensional space, while other groups may only admit a poor representation, which may yield poor results for all groups.
%Minimizing the maximum reconstruction error over the groups, without taking the best possible per-group reconstruction into account,
%may yield poor results.
%More specifically, for fixed rank $d$, the reconstruction error is lower-bounded by the best possible individual reconstruction error, which is achieved by the \svd. 
In view of this \citet{samadi2018price} introduce the \emph{marginal loss}, which accounts for the best possible individual rank-$d$ reconstruction error of any group.
%More details are given %in~\cite{samadi2018price} and 
%in the technical appendix. 
%This makes the minimum of each group's loss zero. 
%For more details on the marginal loss, refer to previous work~\cite{samadi2018price} and the technical appendix.
%The \emph{marginal loss} is defined as: $loss_{\text{marg}}(\bfA,\bfV) \triangleq \sum_{i=1}^d\sigma_i^2(\bfA) - \|\bfA\bfV\bfV^T\|_F^2$. An additional property of this loss function is that it lower bounds the minima of the group-wise errors at the same value (in this case at zero). As will become clear later, this is a useful property for \maxloss, since it ensures that for $|\groups|=2$, we have parity of loss in the optimal solution.
%In this work, we also aim to consider the best possible reconstruction error attainable for any group. 
In the appendix we provide more details on the marginal loss, and we show that its useful properties in the problem studied by~\citeauthor{samadi2018price} do not carry over to our setting, where the marginal loss may even take on negative values. 
\iffalse
\cnote[HM]{This paragraph is OK, but I experimented here with moving it to follow definitions 1 and 2.}

\cnote[AM]{I like the new structure more.}

\cnoteokhm
\fi 


\spara{Formal statement of the problem.} 
We are now in a position to formalize the problem we study. 
%\cnote[HM]{Check the name of problems: define fairsvdextended as  "Singular vectors for multigroup data"}
\begin{problem}[\fairsvdextended]
\label{prob:fairsvd}
Given $\matrixM \in \reals^{m \times n}$ with row partition $\bfA^1, \ldots, \bfA^k$, find $\bfV \in \reals^{m \times r}$ with orthonormal columns such that for all $d \in \{1,\ldots,r\}$:
%the matrix $\bfV_{:d}$ minimizes the quantity
%\cnote[HM]{Here one should use argmin notation; changed to that, hope it is correct.}
\begin{equation}
    \label{eq:max_loss}
    \bfV_{:d} = \argmin_{\bfV \in \reals^{m \times r}}    
 \{ \lossIncremental(\bfA^1,\bfV),\ldots,\lossIncremental(\bfA^k,\bfV)\}. 
%{\lossIncremental(\bfA^1,\bfV_{:d}),\ldots,\lossIncremental(\bfA^k,\bfV_{:d})\}. 
\end{equation}
\end{problem}

%For ease of notation, t
Throughout paper, we refer to the loss in Equation~\ref{eq:max_loss}  as $\maxLArgs{\matrixM}{\bfV}$. 


\iffalse 

In the single-group scenario, one computes the error associated with such a dimensionality-reduction techniques as the \svd by projecting the data of rank $d'>d$ onto the basis formed by the first $d$ singular vectors and then computing the reconstruction error. 
If multiple group are present, it is desirable to minimize the maximum error across all the groups in the data so that 


To formalize our problem, it is now left to specify the loss function measuring the error associated with each group. 
We introduce a \emph{loss function} $\loss: \VV_d \rightarrow \reals$,  


 given a data matrix $\matrixM \in \reals^{m\times n} $ and an associated \emph{loss function}, $\loss: \VV_d \rightarrow \reals$, which computes the error of representing $\matrixM$ by projecting it onto a lower dimensional subspace spanned by $\bfV \in \VV_d$.

\fi 

%\cnote[]{This is nice. Did you also the edit the next part? It refers to maxloss which has not been defined.}

\spara{Computational complexity}. We conclude this section with a note on the computational hardness of \fairsvdextended. We observe that this problem contains the \fairpca problem~\cite{tantipongpipat2019multi} as a special case, when $d=1$. In fact, \citeauthor{tantipongpipat2019multi} prove that when the number of groups $|\groups|$ is part of the input, the problem is \np-hard even for $d=1$, through a reduction from \maxcut. 
Fortunately, as we show next, our problem is polynomially solvable for the case of $|\groups|=2$, and this case will be the main focus of our paper. For $|\groups|>2$, our method may return a non-optimal solution, i.e., the obtained $\bfV_{:d}$ may not be the minimizer for all $d \in \{1,\ldots,r\}$ as Problem \ref{prob:fairsvd} requires. 
In this case, to avoid ambiguity, we will order solutions lexicographically: $\bfV < \bfV'$  if 
$\maxLArgs{\matrixM}{\bfV_{:d}} < \maxLArgs{\matrixM}{\bfV'_{:d}}$ for the smallest possible $d\in\{1,\ldots,r\}$.
%while equality holds for $1,\ldots,d-1$. 
In practice, we show that the the solutions given by our methods
%retrieved by the methods we propose to address 
for the case of more than two groups are consistently close to optimal. 

%\section{Complexity of \fairsvd}


%Tantipongpipat et al. also focus on the case when there are two ($k=2$) groups in the data. This case is polynomially solvable through an SDP relaxation, however at the cost of an extra dimension ($d+1$) \cite{samadi2018price}. However, as we show next, our problem formulation admits an exact polynomial algorithm, for the case of $k=2$. We call this problem \twofairsvd, and we focus on this problem for the majority of this work. 

%\begin{problem}[2-group FairSVD]
%\label{prob:twofairsvd}
%Given matrix $M \in \reals^{m \times n}$ with row partition $M=\{A, B\}$
%, let $r=\min\{\rank(A),\rank(B)\}$
%, find a matrix with orthonormal columns $V=\{v_1,\ldots,v_d\}$, such that the projector obtained as $X=V_{:d}V_{:d}^T$ minimizes \minmaxloss for all $d$.
%$X=V_{[k]}V_{[k]}^T$ is optimal rank$-k$ projection
%for all $V_{[k]}$, where $[k]=\{1,\ldots, k\}$ is the set of the first $k$ indices of the basis vectors in $V$. 
%\end{problem}

%We call this problem \twofairsvd. 
%We also have the following theorem, which we will prove in Section \ref{sec:twofairsvd_algo}.
%\begin{theorem}
%\label{theorem:algo}
%    There exists an algorithm that solves \twofairsvd optimally in polynomial time. 
%\end{theorem}

%We call this problem \twofairsvd. 
%We also have the following theorem, which we will prove in Section \ref{sec:twofairsvd_algo}.

==> inductive_proof.tex <==

The proof relies on an inductive argument and the fact that constraints \ref{constr:h_A} and \ref{constr:h_B} are tight. We show this using the complementary slackness condition of the KKT conditions. 

\textbf{Base case: }For the base case, assume that we are in step $r=1$ of Algorithm \ref{alg:fairsvd}. Denote the right singular vectors of $A$ as $W=\{w_1,\ldots,w_n\}$ and the right singular vectors of $B$ as $U=\{u_1,\ldots,u_n\}$.  

The complementary slackness condition for Problem \ref{prob:fair_eig} states that $\mu_1 h_A(v^*, z^*)=0$ and that $\mu_2 h_B(v^*,z^*)=0$ for an optimal solution $v^* \in \reals^{n}, z^* \in \reals$. 

We distinguish cases for the values of $\mu_1$ and $\mu_2$.

\begin{itemize}[noitemsep,leftmargin=*]
    
\item { $\boldsymbol{\mu}_{\mathbf{1}}\mathbf{=}\boldsymbol{\mu}_{\mathbf{2}}\mathbf{=0}$}. Then both constraints \ref{constr:h_A} and \ref{constr:h_B} are inactive, and the obtained solution is infeasible. 

\item{$\boldsymbol{\mu}_{\mathbf{1}}\mathbf{=0}$ and $\boldsymbol{\mu}_{\mathbf{2}} \mathbf{\neq 0}$.} 
Thus the constraint described by $h_A$ becomes inactive. 
For $r=1$ we have $t_A=\|Aw_1w_1^T\|_F^2$ and $t_B=\|Bu_1u_1^T\|_F^2$, the norms of best rank-$1$ approximations to $A$ and $B$ accordingly. Thus Problem \ref{prob:fair_eig} becomes the problem of minimizing $\|Bu_1u_1^T\|_F^2-\|Bvv^T\|_F^2$ under a unit-norm constraint for $v$. This is a maximum eigenvalue problem, and can be easily solved to give $v=u_1$. Thus, the variable $z$ is set to $z=0$, and $h_B=0$. However, we see that unless $u_1=w_1$ this necessarily violates constraint \ref{constr:h_A}, since $\|Aw_1w_1^T\|-\|Avv^T\| \leq 0$ cannot hold due for vector $v \neq w_1$ (due to optimality of $w_1$). For the case of $u_1=w_1$, $\loss_A(vv^T)=\loss_B(vv^T)$ trivially holds. The argument for the case of $\mu_1 \neq 0$ and $\mu_2 = 0$ is symmetric.


\item $\boldsymbol{\mu}_{\mathbf{1}} \mathbf{\neq 0}$ and $\boldsymbol{\mu}_{\mathbf{2}} \mathbf{\neq 0}$. The complementary slackness conditions $\mu_1h_A(v^*,z^*)=0$ and $\mu_2h_B(v^*,z^*)=0$ imply that $h_A(v^*,z^*)=h_B(v^*,z^*)=0$, and therefore $t_A-\|Avv^T\|_F^2=t_B-\|Bvv^T\|_F^2$ and thus $\loss_A(vv^T)=\loss_B(vv^T)$.

\end{itemize}


\textbf{Inductive hypothesis:} Assume that we are in some step $r$ and it holds that $\loss_A(V_{:r}V_{:r}^T)=\loss_B(V_{:r}V_{:r}^T)$.

\textbf{Inductive step:}  For $r+1$ we have to solve the \faireig problem for $t_A=\|Aw_{r+1}w_{r+1}^T\|_F^2$ and $t_B=\|Bu_{r+1}u_{r+1}^T\|_F^2$. 
Similarly as before, we proceed by case by case analysis. 
We now discern two cases for the values of $\mu_1$ and $\mu_2$. 
\begin{itemize}[noitemsep,leftmargin=*]
\item{$\boldsymbol{\mu}_{\mathbf{1}}\mathbf{=0}$ and $\boldsymbol{\mu}_{\mathbf{2}} \mathbf{\neq 0}$.} 
%$\mu_1 = 0$, $\mu_2 \neq 0$ or ($\mu_1 \neq 0$, $\mu_2=0$). 
%Assume the first condition, since the other one is symmetric. 
Then constraint \ref{constr:h_A} becomes inactive. In step $r$ of Algorithm \ref{alg:fairsvd} we have that $A^c=A(I-V_{:r}V_{:r}^T)$ and $B^c=B(I-V_{:r}V_{:r}^T)$, i.e. $A$ and $B$ lie in the orthogonal complement of the selected basis vectors so far. Since constraint \ref{constr:h_A} is inactive, the solution $v_B^*$ is the maximum eigenvalue of $B$ in that subspace. Denote the associated value of $z$ as $z_B$. If the constraint
\[
\|Aw_{r+1}w_{r+1}^T\|_F^2 - \|A^c v_Bv_B^T \|_F^2 \leq z_B
\]
is satisfied, then $v_B$ is feasible and actually the optimal solution. To see this, observe than any other solution $v^*$ that decreases $h_A$ necessarily increases $h_B$, due to the optimality of $v_B$ for $h_B$. Thus it can only make the minmax objective increase. The case of $\mu_1 \neq 0$ and $\mu_2 = 0$ is symmetric.

\item $\boldsymbol{\mu}_{\mathbf{1}} \mathbf{\neq 0}$ and $\boldsymbol{\mu}_{\mathbf{2}} \mathbf{\neq 0}$.
Both constraints are active. From the complementary slackness condition we see that $h_A=h_B=0$. 
%We set $E_A=\|AW_{:r}W_{:r}^T\|_F^2-\|AV_{:r}V_{:r}^T\|_F^2$ and $E_B=\|BU_{:r}U_{:r}^T\|_F^2-\|BV_{:r}V_{:r}^T\|_F^2$. 
Thus we have
%\begin{align*}
%\|Aw_{r+1}w_{r+1}^T\|_F^2 + E_A - \|A^cv_{r+1}v_{r+1}^T\|_F^2 &\ = z^* \\
%\|Bw_{r+1}w_{r+1}^T\|_F^2 + E_B - \|B^cv_{r+1}v_{r+1}^T\|_F^2 &\ = z^*
%\end{align*}
%From inductive hypothesis we have that $E_A=E_B=E$. Thus 
\[
\|Aw_{r+1}w_{r+1}^T\|_F^2 - \|A^cv_{r+1}v_{r+1}^T\|_F^2 = \|Bw_{r+1}w_{r+1}^T\|_F^2 - \|B^cv_{r+1}v_{r+1}^T\|_F^2 
\]
\end{itemize}


==> introduction_old.tex <==
\section{Introduction}
Low-rank approximation techniques provide dimensionally reduced representations of data by expressing the data matrix as a linear combination of a small number of factors. Such methods are fundamental in machine learning and data science, due to the benefits they offer in terms of scalability, interpretability, and their strong mathematical foundation. 

Among other methods, the singular value decomposition (\svd) holds a central position. A celebrated result states that the first $d$ left or right singular vectors offer the best possible rank-$d$ approximation to a matrix $M$ in terms of Frobenius or spectral norm \cite{eckart1936approximation}. We call this the \emph{consistency} property of the \svd.

In many applications, the rows of a data matrix are divided into two or more groups according to a particular attribute, e.g., gender.  
In such a case, using the top $k$ right singular vectors may not represent every group equally well, potentially resulting in inaccurate or even discriminatory outcomes.
To address these concerns, previous works
~\cite{samadi2018price,tantipongpipat2019multi, song2024socially} have studied the problem of finding a \emph{common} projection onto a subspace that minimizes the worst-case reconstruction error of any group. This problem is typically referred to as \fairpca. 

While effective, previous methods~\cite{samadi2018price,tantipongpipat2019multi, song2024socially} do not ensure the consistency property of the \svd, i.e., given a basis of a subspace, it is not possible to readily obtain a basis of a lower-rank subspace simply by discarding some vectors. 

Building on this line of work, we introduce a \emph{multigroup} low-rank approximation formulation which, in the spirit of the \svd, imposes the consistency property. 
More specifically, given a 
data matrix $\matrixM$ with rows divided into groups $\groups=\{\bfA^1,\ldots,\bfA^k\}$, we look for an orthonormal basis $\bfV$ for a subspace of the column space with the following properties: 1) projecting onto it minimizes the maximum possible error of any group (min-max criterion), 2) is consistent: given the best $r$ vectors, the first $d<r$ vectors from that solution are the best possible solution to the problem of finding $d$ basis vectors. We call such vectors \emph{multigroup singular vectors}.
%The basis vectors in $\bfV$ can be interpreted as the directions where the minimum variance of any group is maximized.
\input{ first_figure}
 Figure \ref{fig:two_figures} illustrates the concept of multigroup singular vectors. 
 \mc{Figure 1 (a) shows the standard singular vectors (in red) and multigroup singular vectors (in green) in synthetic data. While standard singular vectors clearly favor the larger group over the smaller, multigroup singular vectors seek a more balanced representation. 
 }
Figure~\ref{fig:two_figures} (b) instead shows a comparison in the real-world \compas dataset~\cite{dua2019uci}. We consider the partitioning of the data into females and males. 
Projecting onto the multigroup singular vectors leads to a more balanced reconstruction error than projecting onto standard singular values, while giving a similar overall reconstruction error.


We empirically evaluate our method in the task of \fairpca ~\cite{samadi2018price}. We show that it ensures the consistency property while incurring similar reconstruction error to the previous methods~\cite{samadi2018price,tantipongpipat2019multi, song2024socially}. 
In addition, an obvious advantage of the consistency property is that it confers high efficiency and scalability:  we can compute each basis vector efficiently, and once the full-rank basis is computed, we can obtain lower-dimensional representations of any rank by just discarding basis vectors, as for \svd.
This is in contrast to the previous approaches~\cite{samadi2018price,tantipongpipat2019multi, song2024socially} which require solving an independent, computationally challenging problem for any basis dimension. 

The multigroup low-rank approximation problem still presents significant challenges. To ensure the consistency property holds, we construct the $k$-dimensional solution through an iterative process of solving simpler rank-$1$ problems. The more difficult aspect is proving that this procedure also yields the optimal $k$-dimensional result. Notably, we demonstrate that our solution is in fact optimal in the case of two groups in the data. For scenarios with more than two groups, we show that our solutions are empirically close to optimal in practice.
%\cnote{Does our method guarantee that?}


The contributions of this work can be summarized as follows. 
\begin{itemize}[noitemsep,topsep=0pt, leftmargin=10pt]
    \item We formalize the consistent multigroup low-rank approximation problem. 
     \item We give an iterative procedure which selects the best basis vector according to the min-max criterion, and then projects the data onto the orthogonal complement of the previously chosen vectors. The selection of the best basis vector at each iteration represents the main algorithmic challenge that we tackle. 
    \item We theoretically analyze the formulated problems and the proposed algorithms, focusing on the two-groups case, which exhibits interesting properties. 
    \item We describe extensive experiments on real-world datasets to demonstrate the benefits of consistent low-rank approximation over previous work.
\end{itemize}

The rest of this paper is organized as follows. Section \ref{sec:related_work} gives an overview of related work. Section \ref{sec:preliminaries} gives necessary notations and definitions. Section \ref{sec:overview} describes our overall framework. Section \ref{sec:fair_eig} formally introduces the multigroup singular vector problem (\faireig), while Section \ref{sec:algos} proposes algorithms to solve it. We present a theoretical analysis and give an algorithm for a special case in Section \ref{sec:twogroup_analysis}, while Section \ref{sec:experiments} contains our experimental evaluation 
and Section~\ref{sec:conclusion} presents conclusions. 

==> orthonormalization.tex <==


%\section{High Level Algorithm}
\section{Overview of the method}
\label{sec:algo}

In this section we describe the  multigroup dimensionality-reduction method. 

\spara{Preliminary remark.} 
To perform dimensionality reduction, \svd or \pca compute the right singular vectors in the input matrix $\matrixM$.  
One way of obtaining these vectors is by iteratively solving  the following problem:
%At the $i$-th iteration:
\begin{equation}
\label{eq:decomposition}
    \max_{\bfv ; \|\bfv\| = 1} \|\matrixM\bfv\bfv^\top\|_F^2, \quad \mbox{where} \, \bfv \in \bfV_{:i}^{\perp},
\end{equation}
where $i$ indexes the iterations.
\cnote[HM]{$\bfV$ is not defined here!? }
%In \svd, we are given a data matrix $\matrixM$, and we want to compute the singular values and the orthogonal matrices $\bfU$ and $\bfV$ corresponding to the left and right singular vectors. 
In other words, at each iteration, we find the vector $\bfv$ that maximizes the norm of the projection of $\matrixM$, and belongs to the orthogonal complement of the previously found vectors. This is called an \emph{orthonormalization} process. 
%Similarly, the left singular vectors can be obtained through orthonormalization by iteratively projecting the columns of $\matrixM$. 
%Equivalently, one can eigendecomposition of $\matrixM^T\matrixM=\bfV\Lambda\bfV^T$ and accordingly $\bfU$ is obtained from the eigendecomposition of $\matrixM\matrixM^T$. 
% The spectral theorem guarantees the existence of an orthonormal basis which satisfies the above property. In fact, these vectors are the eigenvectors of $\matrixM^T\matrixM$ 
 %and $\matrixM\matrixM^T$
%~\cite{strang2012linear}. 
%\cnote[]{Is this sentence necessary? "The spectral theorem guarantees the existence of an orthonormal basis which satisfies the above property. In fact, these vectors are the eigenvectors of $\matrixM^T\matrixM$ "}
%\cnote[HM]{Changed the title of the paragraph above to clarify that we do not first do classical orthonormalization. }
%\cnoteokhm

\spara{Algorithm description.} We introduce an algorithm for Problem~\ref{prob:fairsvd}  
%\cnote[HM]{Check the names for the algorithm used later.}
that carries out an orthonormalization process while taking groups into account.
%, and is similar in idea to the spectral decomposition (citation needed). 
Before proceeding, we note that while the concept of right singular vectors carries over naturally to the multigroup setting, there is no natural multigroup extension of the left singular vectors, since the rows and not the columns of the data matrix $\matrixM$ are partitioned into groups.
\cnote[HM]{This would need some additional explanation: $M = USV^T$, and the columns of $V$ are the right singular vectors. If $M$ has dimensions $(n,p)$, then $V$ and $V^T$ have dimensions $(p,p)$, so how do the columns of $V$ correspond with the groups? I'm probably misunderstanding something}%, so that data of different groups reside in different subspaces. 
Thus, we are interested in projections of the rows of $\matrixM$ of the form of Equation 
\ref{eq:decomposition}. 
\cnote[HM]{This last sentence I understand.}
\iffalse 
\cnote[HM]{Not quite clear what projections refers to in the last sentence of the paragraph.}
\cnote[AM]{Is it clearer now?}
\cnoteokhm
\fi 
The iterative algorithm for Problem~\ref{prob:fairsvd} works %described 
as follows. 
We solve a rank-$1$ problem to obtain the multigroup singular vector $\bfv_1$. 
Given $\bfv_1$,  we project the groups in $\groups$ onto $\{\bfv_1\}^{\perp}$, the orthogonal complement of $\bfv_1$. We repeat the same process on $\{\bfv_1\}^{\perp}$ to obtain a new vector $\bfv_2$. Repeating this process $d$ times, we obtain an orthonormal basis $\bfV=\{\bfv_1,\ldots,\bfv_d\}$ for a balanced subspace. 

%\cnote[HM]{Modified the order a little bit: first the overall algorithm, then introducing  \faireig formally.}
%\cnote[AM]{Good, I agree its better to give a high-level description first.}
%\cnoteokhm
To implement this procedure we need to be able to solve the following rank-$1$ problem:
%which asks for the vector $\bfv$ defined as:
\begin{equation}
\label{eq:rank_1}
\argmin_{\bfv} \max_{\bfA^i \in \groups} \{ \ssq(\bfA^i) -\|\bfA^i\bfv\bfv^\top\|_F^2\}.      
\end{equation}
We call this problem \faireig, and we consider it in detail in the following section.

The whole iterative process is summarized in Algorithm \ref{alg:fairsvd}. 
%
Step~\ref{step:faireig} of the algorithm corresponds to a call to a subroutine, described in the following sections, that solves the \faireig sub-problem. 
%This subroutine represents a core contribution of this work, and details are provided in the following sections. 
Step~\ref{step:orthcompl} instead illustrates the projection onto the orthogonal complement of the solution vector to the \faireig sub-problem.




%For completeness, in the technical appendix we provide a proof that $\bfV$ is indeed an orthonormal basis. 

\spara{Loss decomposition.}
How good is Algorithm \ref{alg:fairsvd} in minimizing our loss function, $\lossIncremental$? Since our algorithm iteratively produces orthonormal vectors,  Definition~\ref{lemma:total_loss} and a simple inductive argument imply that $\lossIncremental$ for a solution of $d$ dimensions is the sum of $d$ losses of rank-$1$ solutions. Thus, the quality of our solution depends only on our ability to solve a rank-$1$ problem.
Indeed, assume we are in step $r$ of Algorithm \ref{alg:fairsvd}:  we have $\{\bfV\}=\{\bfv_1,\ldots,\bfv_{r-1}\}$, and we seek $\{\bfV'\}=\{\bfV\}\cup \{\bfv\}$ that optimizes $\lossIncremental$. 
Since $\lossIncremental(\bfV')$ can be decomposed as $\lossIncremental(\bfV')=\lossIncremental(\bfV)+\lossOneD(\bfv)$, we are interested in solving a sequence of rank-$1$ problems to find the optimal $\bfV$. In the following sections, we will show that, for the case of two groups, we can in fact solve the rank-$1$ problem optimally, and for the general case we will give an approximate algorithm which works well in practice.
\iffalse
\cnote[HM]{A few additional sentences would be useful here: "we are interested in", but the reader wants to know whether we manage to do this. What about adding something like "We will show that for the case of two groups we can indeed solve the rank-1 problem optimally, and for the general case we will give an approximate algorithm which works well in practice."}
\cnote[AM]{Thanks, I implemented your suggestion.}
\cnoteokhm
\fi 

\spara{Complexity.} The overall time complexity is $\mathcal{O}(d\ell)$, where $\mathcal{O}(\ell)$ is the complexity of \faireig. 

%\begin{problem*}[\faireig]
%\label{prob:fair_eig}
%    Given matrices $\{\bfA^1,\ldots,\bfA^k\}$, $\bfA^i \in \reals^{m_i \times n}$, find $\bfv$ such that:
%    \[
%    \argmin_{\bfv} \max_{i \in \groups} \{ \ssq(\bfA^i) -\|\bfA^i\bfv\bfv^T\|_F^2\} 
%    \]
%\end{problem*}
%\cnote[HM]{In the notation $A^i w^i_r w_r^{iT}$ is $w^i_r$ a single vector or a set of vectors?}{}

%This completes the description Algorithm \ref{alg:fairsvd}. 

%\cnote[HM]{We should state what are the arguments of \faireig and what it returns.}{}



\begin{algorithm}[t!]
\caption{Multigroup Orthonormalization}
    \label{alg:fairsvd}
	\textbf{Input:} %$\matrixM \in \reals^{m\times n}$, 
     matrices $\{\bfA^1,\ldots, \bfA^k\}$.   %a set of $\reals^{m_i \times n}$  matrices. \\
	%\textbf{Output:} $\bfV\in \reals^{n\times d}: \bfV^T\bfV=\matrixI_d$.
	\begin{algorithmic}[1]
     \STATE Initialize $r\gets 1$, $V \gets \emptyset$
        \WHILE{$r<=d$}
        \STATE \label{step:faireig} $\bfv_r\gets$ \faireig($\bfA_1,\ldots,\bfA_k$)
        \STATE \label{step:orthcompl} $\bfA_i \gets \bfA_i - \bfA_i\bfv_r\bfv_r^\top$  
        \STATE $\bfV \gets \bfV \cup \bfv_r$
        \STATE $r \gets r+1$
        \ENDWHILE
	\end{algorithmic}
	{\bf return} $\bfV$
\end{algorithm}

\iffalse

\spara{Quantifying the price of balance.}
We conclude with some discussion on singular values. 
For the \svd, we have $\sigma_i(\bfA)=\|\bfA\bfw_i\bfw_i^\top\|_F$, when $\{\bfw_1,\ldots,\bfw_d\}$ are the first $d$ right singular vectors of $\bfA$.
%Recall the equivalence $\sigma_i(\matrixM)=\|\matrixM\bfw_i\bfw_i^T\|_F$, where $\bfw_i$ is the $i$-th right singular vector of $\matrixM$, i.e. 
Thus the $i$th singular value reflects the norm of the projection of $\matrixM$ onto the $i$th optimal axis, which is orthogonal to the previous ones. 

We present a similar concept for \fairsvd. Assuming the optimal solution $\bfV^*=\{\bfv_1^*,\ldots,\bfv_d^*\}$ to \fairsvd, we define the values $\phi_i(\matrixM)$ as
\[ 
\phi_i(\matrixM) = \|\matrixM\bfv_i^*{\bfv_i^*}^\top\|_F
\].
That is, $\phi_i(\matrixM)$ is the norm of the projection of $\matrixM$ onto the optimal $i$-th balanced axis.
%As we can see, the incremental loss comprises of two terms, $\sum_{i=1}^d \sigma_1^2(A_i)$ and $\sum_{i=1}^d\|Av_iv_i^T\|_F^2$. The first term describes the best possible representation of $A$ within the fair subspace of $V$.  We will call the difference between the norm of the best rank-$k$ representation of $A$, given by $\sum_{i=1}^d\sigma_i^2(A)$ and the best possible representation within the fair subspace $V$, as the \emph{price of consistency} for $A$.
%\begin{definition}[Price of consistency]
%\[
%\sc{PoC}(A)\triangleq \sum_{i=1}^d\sigma_i^2(A) - \sum_{i=1}^d \sigma_1^2(A_i)
%\]
%\end{definition}
%On the other hand, the term $\|AV^*{V^*}^T\|_F^2$ describes the norm of the optimal fair projection of $A$ onto $d$ dimensions. 
This has an interesting interpretation: the term 
\[
   \sum_{i=1}^d\sigma_i^2(\matrixM) -  
      \sum_{i=1}^d\phi_i^2(\matrixM)
\]
describes how much we lose in terms of overall accuracy by considering a balanced approach for \svd. We call this the \emph{price of balance}. % and we study this quantity in the experiments section.  
\cnote[HM]{Do we refer to this (excellent) concept in the sequel?}
\fi

==> proof_of_lemma2.tex <==

\subsection{Proof of Lemma \ref{lemma:equal_loss}}

Recall that for the two-group case, we assume that $M \in \reals^{m\times n}$ is partitioned into two groups $A \in \reals^{m_a \times n}$ and $B \in \reals^{m_b \times n}$. 

\begin{problem}[2-group \faireig]
\label{prob:twofaireig_optimization}
{\begin{align}
\min_{v \in \reals^n, z \in \reals} \, \, z & \nonumber \\
\text { s.t. }  & \label{constr:h_A} \ssq(A)- \|Avv^T\|_F^2 \le z\\
     & \label{constr:h_B} \ssq(B)- \|Bvv^T\|_F^2 \le z\\
     & \label{constr:norm} \|v\|_2^2=1
\end{align}} 
\end{problem}

As before, we define the following two constraint functions: $h_A(\bfv) = \ssq(A) - \|A\bfv\bfv^T\|_F^2$ and $h_B(\bfv) = \ssq(B) - \|B\bfv\bfv^T\|_F^2$,
which represent the inequality constraints \ref{constr:h_A} and \ref{constr:h_B} with associated KKT multipliers $\mu_A \in \reals$ and $\mu_B \in \reals$. 


%Before going into the theorem, first we describe the following property that will help us prove theorem \ref{theorem:equal_loss}. 

%\begin{property}[Optimality of \svd]
%\label{property:optimality_svd}



\begin{proof}
The proof relies on the fact that constraints \ref{constr:h_A} and \ref{constr:h_B} are tight. We show this using the complementary slackness condition of the KKT conditions. 

Assume that we are in step $r$ of Algorithm \ref{alg:fairsvd}. 
%Denote the right singular vectors of $A$ as $W=\{w_1,\ldots,w_n\}$ and the right singular vectors of $B$ as $U=\{u_1,\ldots,u_n\}$.  
The complementary slackness condition for Problem \ref{prob:fair_eig} states that $\mu_A h_A(v^*)=0$ and that $\mu_B h_B(v^*)=0$ for an optimal solution $v^* \in \reals^{n}$. 

We distinguish cases for the values of $\mu_A$ and $\mu_B$.

\begin{itemize}[noitemsep,leftmargin=*]
    
\item { $\boldsymbol{\mu}_{\mathbf{A}}\mathbf{=}\boldsymbol{\mu}_{\mathbf{B}}\mathbf{=0}$}. Then both constraints \ref{constr:h_A} and \ref{constr:h_B} are inactive, and the obtained solution is infeasible. 

\item{$\boldsymbol{\mu}_{\mathbf{A}}\mathbf{=0}$ and $\boldsymbol{\mu}_{\mathbf{B}} \mathbf{\neq 0}$.} 
We show that any solution that satisfies these constraints, either achieves equal loss, or is infeasible.
%$\mu_1 = 0$, $\mu_2 \neq 0$ or ($\mu_1 \neq 0$, $\mu_2=0$). 
%Assume the first condition, since the other one is symmetric. 
Since $\mu_A=0$, then constraint \ref{constr:h_A} becomes inactive. In step $r$ of Algorithm \ref{alg:fairsvd} we have that $A_r=A(I-V_{:r-1}V_{:r-1}^T)$ and $B_r=B(I-V_{:r-1}V_{:r-1}^T)$, i.e. $A$ and $B$ lie in the orthogonal complement of the selected basis vectors so far. If $r=1$, then $A_1=A$ and $B_1=B$. Since constraint \ref{constr:h_A} is inactive, the solution $v_B^*$ is the dominant eigenvector of $B$ in the subspace $V_{:r-1}^{\perp}$ (for $r=1$ it is simply the maximum eigenvalue). Denote the associated value of $z$ as $z_B$. 
\[
z_B= \ssq(B_r) - \|B_rv_Bv_B^T\|_F^2 = 0
\]
%We can see that 
%\[
%\|B^cv_Bv_B^T\|_F^2 = \sigma_{max} (B^c).
%\]
%By invoking property \ref{property:optimality_svd}. We have that
%\[
%\|Bu_ru_r^T\|_F^2 - \|B^cv_Bv_B^T\|_F^2 = \|Bu_ru_r^T\|_F^2 -\sigma_{max}(B^c) %\leq 0
%\]
Now consider the case that the solution is feasible and $h_A < h_B$. We will see that this leads to a contradiction. 
Based on the above assumption we have that 
\begin{align*}
    \ssq(A_r) - \|A_r v_Bv_B^T \|_F^2 - z_B  & < \\
    \ssq(B_r) - \|B_rv_Bv_B^T\|_F^2 - z_B    & = 0 
\end{align*}
Which leads to $\ssq(A_r) - \|A_r v_Bv_B^T \|_F^2 < 0$. However this would imply that \loss for $A$ is negative, which is in violation of Observation \ref{obs:minzero}. Thus $h_A < h_B$ leads to a contradiction, and it must also hold that $h_A-z_B=0$ for the solution to be feasible. The case of $\mu_A \neq 0$ and $\mu_B = 0$ is symmetric.

\item $\boldsymbol{\mu}_{\mathbf{A}} \mathbf{\neq 0}$ and $\boldsymbol{\mu}_{\mathbf{B}} \mathbf{\neq 0}$.
Both constraints are active. From the complementary slackness condition we see that $h_A=h_B=0$. 
%We set $E_A=\|AW_{:r}W_{:r}^T\|_F^2-\|AV_{:r}V_{:r}^T\|_F^2$ and $E_B=\|BU_{:r}U_{:r}^T\|_F^2-\|BV_{:r}V_{:r}^T\|_F^2$. 
Thus we have
\[
\ssq(A_r) - \|A_rv_{r}v_{r}^T\|_F^2 - z= 0 
\]
\[
 \ssq(B_r) - \|B_rv_{r}v_{r}^T\|_F^2 -z=0
\]
\end{itemize}
which implies that 
\[
\ssq(A_r) - \|A_rv_{r}v_{r}^T\|_F^2=\ssq(B_r) - \|B_rv_{r}v_{r}^T\|_F^2
\]
\end{proof}

